Engaging with Children's Artwork in Mixed Visual-Ability Families

We present two studies exploring how blind or low-vision (BLV) family members engage with their sighted children's artwork, strategies to support understanding and interpretation, and the potential role of technology, such as AI, therein. Our first study involved 14 BLV individuals, and the second included five groups of BLV individuals with their children. Through semi-structured interviews with AI descriptions of children's artwork and multi-sensory design probes, we found that BLV family members value artwork engagement as a bonding opportunity, preferring the child's storytelling and interpretation over other nonvisual representations. Additionally, despite some inaccuracies, BLV family members felt that AI-generated descriptions could facilitate dialogue with their children and aid self-guided art discovery. We close with specific design considerations for supporting artwork engagement in mixed visual-ability families, including enabling artwork access through various methods, supporting children's corrections of AI output, and distinctions in context vs. content and interpretation vs. description of children's artwork.

==> cuts.tex <==
\section{Intro}

%But the visual nature of common children's art creations, such as drawings and paintings, makes it challenging for Blind or Low Vision (BLV) parents or relatives to engage with the artwork in an equivalent manner as sighted family members.

%Technology solutions in this space have turned to tactile representations of artwork \cite{Butler_MultiSensory, Holloway_MakingSenseOfArt}, improvements in descriptions \cite{Morris_RichRepresentations}, and multimodal approaches \cite{Cavazos_MultiModalArtA11y}. There has also been a body of research conducting formative and technology evaluation studies in mixed ability settings \cite{Storer_Branham, Park_AllAboutPictures_2023}. But a gap remains in understanding practices discussing children’s visual creations in Mixed Visual Ability Families (MVAFs). 

% ---

% Our first study included 14 BLV family members and identified the perspectives of BLV relatives when interacting with children through their artwork. Our second study included five groups of BLV family members \textit{and} their children, focusing on the children's perspectives and observing the child-relative dynamic surrounding their artwork. Both studies included semi-structured interviews and gathered feedback about AI interpretations of children’s artwork, and the second study utilized design probes with in-person relative-and-child groups to explore non-visual art representations preferences. Conversations and observations during these studies were recorded, transcribed, and then iteratively coded to reach a set of themes concerning current practices and underlying motivations, desired information about artwork, and responses to actual or potential technology.

% \section{RW}

\section{Study 2 Findings}

% When children share their artwork with BLV family members, they tend to include three inter-related attributes: the \textit{context}, the \textit{content}, and a \textit{narrative}. The context includes the inspiration for the art, where it was created, if it was co-created with another person (a sibling, a teacher), \textit{etc.} Content refers to characteristics of the artwork itself, such as color, shapes, and objects. And the narrative includes \textit{the personal meaning} of the art---which could be the underlying story of a scene or simply the use of the child's favorite crayon or the BLV adult's favorite color. 

% We discovered two aspects of what children share about their artwork to their BLV family member: \textit{context} and \textit{content}. Context included what inspired the art, where the art was created, and if the art was created with another person (a sibling, a teacher). Content included characteristics of the artwork that children shared with their BLV family members, highlighting what was important to the child about the artwork (\textit{e.g.}, use of the child's or BLV adult's favorite colors).

% Children always provided context when describing their art to a BLV family member during the sessions, and conveying context was just as important as the description of the art itself. As an example, P6’s son began his description of a drawing (Figure \ref{CountryBallsAndFlowers}) by saying, \textit{``I used to watch this YouTube channel. It had country balls in it, and they were fighting, and I got really interested in it. So I drew the poster. It's still in progress.''}

\section{Discussion_Revised}

% Affirming Li \textit{et al.} \cite{Li_UnderstandingVisualArtsExperiences}, we find that  BLV individuals typically ask their sighted peers for descriptions of visual art. Our findings revealed that BLV family members' first practice when exploring their children's artwork was to ask their children to describe the work. However, for the BLV individual, the value of learning about their children's artwork was in facilitating an emotional connection through understanding their children's intentions behind the creation, rather than merely understanding the content of the artwork itself. However, the latter was also important. Some of our participants who sought details about the artwork itself did so through exchanges with their children or other sighted adults to gauge their children's developmental milestones. Here, we extend Li et al.'s \cite{Li_UnderstandingVisualArtsExperiences} findings about BLV individuals' motivations to understand visual art to include emotionally connecting with their children and tracking children's developmental milestones.

% Regarding the information BLV family members wanted to access about their children's artwork, our studies showed that they value the children's descriptions above other nonvisual representations. Indeed, even a few BLV family members did not care to learn about specific aesthetic details of the child-created work; this differed from findings in prior research, which mostly focused on adult-created art in museums or activity settings \cite{Li_UnderstandingVisualArtsExperiences, Asakawa_IndependentMuseumExperience}. When BLV family members did want descriptive characteristics, they were curious about the aesthetic quality of the work (colors, balance across the page, techniques used) to help them understand their children's development or to appreciate the effort their children put into the art. Additionally, if BLV family members had an artistic background or held personal preferences about art, conversing with their children about aspects such as color became more important for them. Our findings support prior work in participants' preferences for accessing artwork \cite{Ahmetovic_TouchScreenExplorationOfArtwork, Li_UnderstandingVisualArtsExperiences}, specifically in that BLV family members enjoy both audio and tactile descriptions of their children's work.

% We also found that most BLV family members did not use descriptive tools, such as \textit{Be My Eyes} (including \textit{Be My AI}) or \textit{Seeing AI}, in their artwork-based interactions with their children. BLV family members described that tactile modes were not easily available for families to represent their children's drawings, outside of specific crafts materials such as Wikki Stix, string, or beads. However, we discovered that many BLV family members were excited by the idea of using both AI-generated descriptions and tactile representations when understanding their children's work, supporting Zhang et al.'s \citet{Zhang_StoryBuddy} findings of parents viewing technologies as a means to promote parent-child interactions. 

% Children's reactions to AI descriptions of their artwork were mixed. The children in our studies were curious about AI interpretations of their work but want to play an active role in correcting AI descriptions when they are incorrect. To our knowledge, this is the first work that captures children's perspectives on AI descriptions in support of their BLV family members.

\subsection{Design Implications}

%Drawing on our findings and prior work \cite{importance_for_early_development_2024, Lynch_2012, Rymanowicz_2021, how_parents_can_help_2024, Li_UnderstandingVisualArtsExperiences, Holloway_MakingSenseOfArt, Phutane_2022, Lee_ImageExplorer, XuTeslaTouchCHI2011, Stangl3DPrintIDC14, Ahmetovic_TouchScreenExplorationOfArtwork, Bae_TouchingInformation}, 

% \textit{Enable temporal flexibility.} BLV family members desired autonomy in using nonvisual representations of their children's artwork before, during, or after their interaction with their children. For example, a technology could be leveraged by a BLV individual to understand artwork prior to engaging with their child in order to specific questions about the artwork. Alternatively, they could use technology to recall details of an artwork after an interaction with their child and reflect on that bonding moment with their child.

% \textit{Retain context from the child.} Technology should support understanding the child's intentions and motivations for creating an artwork, along with the setting where the art is created, which is important to both BLV family members and their children. For example, BLV family members might use a mobile application that stores images of the artwork along with contextual information, and upon scanning the same artwork again the application also reminds them of the original context.

% \textit{Make DIY tactility easier for families.} BLV adults and children enjoy tactile explorations of visual work, shown by our studies as well as prior work \cite{Holloway_MakingSenseOfArt, Phutane_2022}. But converting a visual image to a tactile representation is challenging, and fabrication systems such as 3-D printers can be expensive and impractical. There is a need for simpler, more accessible methods to help children convert their visual artwork into tactile forms. Tactile materials expressly devoted to this purpose might be created, such as a tool that can trace over artwork outlines and insert beads on top of the outlines. 
% % squeeze tubes that allow outlining drawings in elevated glue-like substances.

% \textit{Support ``hand-guiding and explaining'' when designing multimodal solutions.} While considerable prior work points to multimodal explorations as a good solution for understanding visual arts \cite{Phutane_2022, Li_UnderstandingVisualArtsExperiences, Ahmetovic_TouchScreenExplorationOfArtwork}, we recommend supporting an experience similar to hand-guiding and explaining, which is a common and valued practice between BLV family members and their children when exploring tactile work together. For example, a tactile system with inbuilt salience clues could guide the BLV family member towards important parts of the tactile art to explore, similar to what \citet{Nair_ImageAssist} created for touchscreens.

% \textbf{Supporting co-creation.} Beyond assessment and interpretation, we found a desire to support co-creation with the child. Here, tools could <fill in>. 

%For the during, the overarching concern was that its potential value of technology was not commensurate with its potential distraction and taking away from the family member-child moment.  



\subsection{Ai-based guidelines}

%For example, a system could compare artwork descriptions from multiple AI models, and output an aggregated description with confidence scores about each component of the final output.
